SMT Sampling via Model-Guided Approximation

We investigate the domain of satisfiable formulas in satisfiability modulo theories (SMT), in particular, automatic generation of a multitude of satisfying assignments to such formulas. Despite the long and successful history of SMT in model checking and formal verification, this aspect is relatively under-explored. Prior work exists for generating such assignments, or samples, for Boolean formulas and for quantifier-free first-order formulas involving bit-vectors, arrays, and uninterpreted functions (QF_AUFBV). We propose a new approach that is suitable for a theory T of integer arithmetic and to T with arrays and uninterpreted functions. The approach involves reducing the general sampling problem to a simpler instance of sampling from a set of independent intervals, which can be done efficiently. Such reduction is carried out by expanding a single model - a seed - using top-down propagation of constraints along the original first-order formula.

==> discussion.tex <==

\section{Model-approximation for additional theories}\label{appendix:additional-theories}
In this work, we chose to solve the model-guided approximation problem (and, consequently, instantiate the sampling framework) for two pairs of theories: $T=\Tmia,T'=\Tic$ and $T=\Tamia,T'=\Taic$.
We chose to sample from $\Tmia$ and $\Tamia$ because, on the one hand, they are commonly used in formal reasoning about software\BC{add citations}; and, on the other hand, to the best of our knowledge, no existing solver can efficiently sample from their solution space.
As to $\Tic$ is a convenient lightweight theory where both satisfiability and sampling are straightforward.

% In addition to the two instantiations presented in the paper, 


% In our work, we chose to sample from interval theories since the focus of our work is model-approximation rather than efficient sampling procedures for the theory $T'$.
% In our work, we chose to sample intervals because the interval domain allows for a simple sampling procedure, while being expressive enough to capture large sets of models in practice.
However, there are several other directions for additional instances of MGA that we consider as future work.
For example, for the rule-based approach of \cref{subsec:rules}, if we were to keep only the rule for multiplication, the result would be a formula in $\Tlia$, instead of $\Tic$.
This formula could then be sampled using a specialized sampling procedure for $\Tlia$, such as~\cite{Meister_Clauss_2020}.

As another example, in cases where intervals, or even general linear formulas, do not make a good under-approximation, additional constraints can be allowed.
For example, the constraint $v\%c=0$, which states that the value of variable $v$ should be divisible by the constant $c$, cannot be under-approximated well using an interval.
However, if we extend $\Tic$ with constraints of this form, we can express this constraint without losing information and without sacrificing the efficiency of the sampling technique (intervals could be sampled at fixed distances). 

Finally, extending our ideas to bit-vectors and reals also seems possible with a rule-based approach similar to that of~\cref{subsec:rules}.
% However, the rules would have to be sensitive to the particular 

% Bit-vector
% Reals

% \subsection{Other applications for model-approximation}

==> eval-with-1-epoch.tex <==
All experiments were run on a 64-core (128-thread) AMD~EPYC~7742 based server
with 512GiB of memory.

Our aim in the evaluation is to answer three questions: \BC{turn this into framed text instead of enum?}
\begin{enumerate}
    \item \textbf{Expendability} Which algorithm is the most effective in expanding a single seed?\BC{I don't think we have used this terminology before, though}
    \item \textbf{Quantity} How efficient is \MeGASampler, in terms of the number of samples?
    \item \textbf{Quality} How efficient is \MeGASampler, in terms of the quality of samples?
\end{enumerate}

\paragraph{RQ1: Expendability}
% How large are the intervals we get in practice using the model-approximation algorithms for $\Tmia$ and $\Tamia$.
% How many solutions does an $m$-approximation $\varphi'$ of $\varphi$ has, when obtained using the rule-based algorithm
To answer RQ1, we run both algorithms on the same seed for x minutes and counted the number of samples they were able to obtain.
This experiment was designed to evaluate the MGA algorithm (section 4), as opposed to the sampling algorithm (section5). to do that, we compared only one epoch, and on the same seed. 

Both \MeGASampler and \SMTSampler are based on the concept of expanding a single seed into a large set of samples using limited investment of resources.
In \MeGASampler this is done using MGA (in our case, creating intervals) and in \SMTSampler by applying mutations to the seed and combining them.
In order to compare the ability of the two algorithms to extend the seed, we performed the following experiment:
For each benchmark, we obtained a single seed via a solver, passed it on to both algorithms, and gave both a fixed amount of time in order to expand it and sample as much as possible.
All restrictions on sampling have been removed: in \MeGASampler you can sample as many as you want from the intervals, regardless of their size,
And in \SMTSampler mutations can be combined up to an unbounded depth.

\paragraph{RQ2: Quantity}
\input{eval-table}
%For a deeper look into the performance of the method, 
We perform a case-by-case
comparison between both variants of \MeGASampler and \SMTSampler.  We compute
the ratio between the number of samples generated by \MEGA on each benchmark to
that of \SMTint, and the same for \MEGAb; we then plot the results in descending
order on a logarithmic scale, shown in \cref{fig:eval-plot-num-samples}.
%We also consider the best result among \MEGA and
%\MEGAb \textit{vs.\@} the same baseline.

\paragraph{RQ3: Quality}


==> evaluation.tex <==
We have developed \MeGASampler as an open-source tool, written in \Cpp
and \textsc{Python}. It utilizes the Z3~\cite{DeMoura:2008} solver,
which natively supports all functionality required by \MeGASampler.

We compare three samplers: \MeGASampler with either blocking or random initial
assignments, and a variant of \SMTSampler which was ported from bit-vector logic
to integer logic. The latter was constructed by modifying the original
\SMTSampler implementations as follows.  \SMTSampler is built upon three
operations: transforming the solution into a set of conditions that it
satisfies, finding similar solutions by negating one of these conditions, and
combining the resulting solutions to generate new solution
candidates. Therefore, porting to a different logic requires translating these
operations to fit that logic. For bit-vectors, \SMTSampler used conditions of
the form ``bit \(i\) in vector \(v\) is set'', and combined solutions by
applying a bitwise~or operation to mutated values. For the integer domain, we
chose to consider the entire assignment as a condition, \ie ``integer \(x\) is
equal to value \(n\)'', and used addition as the integer analogue for combining
mutations.

All experiments were run on a 64-core (128-thread) AMD~EPYC~7742 based server
with 512GiB of memory. Each execution utilized a single core, until either a
time limit of 30 minutes was reached, or 1000000 unique samples were
generated. Additionally, each epoch was limited to 10 minutes, to prevent the
samplers from getting stuck on a single seed.

As noted in previous work~\cite{Dutra:2018}, the number of unique solutions
generated is an incomplete metric, which may not represent the samples' coverage
of the solution space. The authors proposed an alternative coverage metric,
hypothesizing that the inner nodes of the formula abstract syntax tree~(AST)
offer higher-level information than just the leaf variables nodes. We have
ported this metric from bit-vector logic to integer logic: each node of sort
Bool represents 1 bit, and each node of sort Int represents 64 bits (\ie the
metric considers only the lower 64 bits of each arbitrary-size integer). The
coverage metric is the ratio of bits that have received both 1 and 0 among the
set of samples. Note that the maximum score using this metric is not necessarily
100\%, because, naturally, some bits are restricted by the input formula and can
only take one of the values.

We performed tests on benchmarks from SMT-LIB~\cite{Barrett:2021}, using the
problems in logics QF\_LIA and QF\_NIA\footnote{The ``interesting'' operation in
  $\Tnia$ is multiplication; most benchmarks in this directory are actually in
  $\Tmia$, which is supported by \MEGASampler.}, as array problems in QF\_ALIA.
Some of the benchmarks represent real-world problems collected by the SMT-LIB
authors, including formulas used for software verification taks, such as
formulas originating in the \textsc{AProVE}~\cite{Giesl:2004} and
\textsc{VeryMax}~\cite{Borralleras:2017} termination analysis tools. Other
benchmarks are synthetic, designed to stress SMT solvers.

We have discarded benchmarks which were inappropriate for the evaluation,
including benchmarks which were marked as unsatisfiable or unknown, as well as
benchmarks for which we could not obtain at least 100 samples by any of our
tested techniques. As we are not evaluating SMT solvers, benchmarks for which
finding a single solution took more than one minute were also discarded. Our
implementation does not support several array features: array equality, and
multi-dimensional arrays\footnote{\SMTSampler does not support multi-dimensional
  arrays either}, therefore we weakened array benchmark files by removing array
equalities. We randomly selected 15 benchmark files as a representative sample
of each directory with a sufficient number of files. Applying these criteria
yielded an evaluation set of 30 benchmark directories (450 files), 4 of which
are in QF\_NIA, 2 in QF\_ALIA, and the rest are in QF\_LIA.

\begin{paragraph}{Limitations of the evaluation.}
  There are some notable limitations to this methodology. Neither of the
  implementations is perfectly tuned; parts of \MeGASampler use \textsc{Python},
  which is inherently slower. \SMTSampler was not designed to work on integers,
  and the modification may not be suitable or optimal. There are several
  parameters controlling sampling behaviors in both implementations, \eg
  mutation depth in \SMTSampler or maximum sample number per epoch in
  \MeGASampler, which were not explored in this work. Different selections for
  these parameters, as well as other experimental parameters such as time limit
  and inputs, may impact the results. There may be other coverage metrics, and,
  for particular uses, metrics other than coverage may better characterize
  ``successful'' sampling.
\end{paragraph}

\input{eval-table}
%
\subsection{Results}
\cref{fig:mega-table} shows the results of the executions, broken down by origin
directory.  For each set of benchmarks, we computed the average number of
solutions, number of epochs, and attained coverage.  The first two columns show
the number of variables and the depth of the formula AST. The columns titled
\MEGA report measurements for the random-based \MEGASampler, \MEGAb---for the
blocking \MEGASampler, and \SMTint---for \SMTSampler retrofitted for the integer
domain. The column labelled \#SMT is the number of MAX-SMT calls during the
run. This value is only presented for \SMTSampler, as in \MeGASampler the number
of MAX-SMT calls is exactly the number of epochs.  Bold indicates the highest
value in each rubric.  Results are aggregated per top-level directory; a more
detailed breakdown is included in \cref{appendix:results-full}.

Overall, both variants of \MeGASampler are capable of obtaining tens of
thousands of solutions.  Also, the coverage of the solutions is often
significant: 44.0\% on average for the random variant and 46.4\% on average for
the blocking variant. This is roughly comparable to \SMTSampler, which produced
a coverage of 45.9\% on average. The amalgamation of the \MeGASampler variants,
where for each benchmark the result with the better coverage is chosen, gives an
average coverage of 55.2\%. \SMTSampler does have an advantage in the total
number of unique solutions produced; however, the coverage metric indicates that
\MeGASampler produces more varied samples.  When considering the number of
solutions generated in each benchmark, \SMTSampler and \MeGASampler obtain
pretty similar results; each gains the highest number in about half the
benchmarks.  Notably, there are several cases where \SMTSampler was able to
reach a very large number of samples, even reaching the sample limit, while
\MeGASampler is far behind. In other cases, the situation is reversed.
Curiously, in both benchmarks where a method has hit the sample limit, it failed
to achieve the highest coverage as well.  However, when considering the coverage
these methods obtain overall, there is a clear advantage to \MeGASampler: in 26
out of 30 cases, the highest coverage is obtained by one of the \MeGASampler
variants.  From within the two variants of \MeGASampler neither has a clear
advantage.

There are some trends that are visible in \cref{fig:mega-table}.  As expected,
\SMTSampler is more sensitive than \MeGASampler to the cost of MAX-SMT
calls. While both methods require MAX-SMT calls to obtain the initial seed,
\MeGASampler is able to generate better samples from it, as is seen for example
in the `leipzig' benchmark, where the samplers were only able to make few
MAX-SMT calls, which severly limited \SMTSampler. % This is also visible in the
% `convert' benchmark, and, to a lesser
% extent, in the `bofill' and `unbd-sage' benchmarks, where \MeGASampler was
% able to extract more solutions while making an equivalent or significantly
% smaller number of SMT-MAX calls. Conversly, in instances where \SMTSampler was
% able to make a large number of MAX-SMT calls, \SMTSampler was able to obtain
% better quality results, as in the `CAV2009/10-vars' and `15-vars'
% benchmark. Interestingly, in these benchmarks it produced less results than
% \MeGASampler; as hypothesized, a large number of samples does not always imply
% increased coverage, since many of the benchmarks feature one or more
% unconstrained variables. The situation was reversed in the `slacked' variant
% of those benchmarks.
\MeGASampler seems well-suited to QF\_NIA problems, with the blocking variant in
particular showing excellent performance. In the QF\_ALIA problems, we see that
the SMT calls were relatively cheap, so \SMTSampler was able to obtain a large
number of solutions; however, the coverage of the solutions obtained by
\MeGASampler was better.

\begin{figure*}[t]
\centering
\ifwithplots
  \input{gfx/cactus-plot-num-samples}
  \vspace{-0.5cm}
\else
  \begin{tabular}{l}
  \includegraphics[width=5cm]{gfx/thumb/graph-1a.png}
  \includegraphics[width=5cm]{gfx/thumb/graph-1b.png}
  \includegraphics[width=5cm]{gfx/thumb/graph-1c.png} \\
  (thumbnails used due to \texttt{\textbackslash withplotsfalse})
  \end{tabular}
\fi
  \caption{A comparison of the number of samples generated by \MeGASampler, relative to those from \SMTSampler.
  The plots show ratios per single benchmark, in descending order,
  comparing each of two variants of \MeGASampler to \SMTSampler,
  as well as the maximum between them.
  }
  \label{fig:eval-plot-num-samples}
  \vspace{0.5cm}
\end{figure*}

\begin{figure*}[t]
\centering
\ifwithplots
  \input{gfx/cactus-plot-coverage}
  \vspace{-0.5cm}
\else
  \begin{tabular}{l}
  \includegraphics[width=5cm]{gfx/thumb/graph-2a.png}
  \includegraphics[width=5cm]{gfx/thumb/graph-2b.png}
  \includegraphics[width=5cm]{gfx/thumb/graph-2c.png} \\
  (thumbnails used due to \texttt{\textbackslash withplotsfalse})
  \end{tabular}
\fi
  \caption{A similar comparison, but for the coverage metric.}
  \label{fig:eval-plot-coverage}
  %\vspace{0.5cm}
\end{figure*}

For a deeper look into the performance of the method, we perform a case-by-case
comparison between both variants of \MeGASampler and \SMTSampler.  We compute
the ratio between the number of samples generated by \MEGA on each benchmark to
that of \SMTint, and the same for \MEGAb; we then plot the results in descending
order on a logarithmic scale, shown in \cref{fig:eval-plot-num-samples,fig:eval-plot-coverage}.  We also consider the best result among \MEGA and
\MEGAb \textit{vs.\@} the same baseline.  The same process is repeated for the
coverage metric defined in \cref{sec:eval}.  While obtaining the maximal result
would require double the CPU time, the improvement in coverage far surpasses
that of each variant alone and may well be worth the extra work.  The reason is
that for some formulas, we have found that the addition of blocking constraints
slows down the seed generation significantly, leading to a smaller number of
epochs.  For the formulas in which this did not occur, the blocking does improve
coverage by striving to cover fresh areas of the space.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> gfx/block-diagram.tex <==

\begin{tikzpicture}[>=stealth]
  \node(input) {$\varphi$};
  \node(input-m)[below=of input] { $m$ };
  \node(toslice)[draw, right=of input] { ToSlice };
  \node(strengthen-1)[draw, right=1.5cm of toslice, yshift=5mm] 
    { Strengthen$^{T}_{T'}$ };
  \node(strengthen-2)[draw, below=2mm of strengthen-1] 
    { Strengthen$^{T}_{T'}$ };
  \node(dotdotdot)[below=0 of strengthen-2, yshift=4pt] { $\vdots$ };
  \node(strengthen-n)[draw, below=2pt of dotdotdot] 
    { Strengthen$^{T}_{T'}$ };
    
  \node(bigand)[draw, right=1.5cm of strengthen-1, yshift=-5mm]
    { $\bigwedge$ };
    
  \node(output)[right=of bigand] {$\widehat{\varphi}$};
  
    
  \draw[->] (input) -- (toslice);
  \draw[->] (input-m) -- (toslice);
  \draw[->] (toslice) -- node[above] {$\xi_1$} (strengthen-1);
  \draw[->] (toslice) -- node[below] {$\xi_2$} (strengthen-2);
  \draw[->] (toslice) -- node[below] {$\xi_n$} (strengthen-n.170);
  \draw[->] (input-m) -- +(0,-9mm) -| (strengthen-n);
  \draw[->] ($ (input-m) + (0,-9mm) $) -| (strengthen-2.-45);
  \draw[->] ($ (input-m) + (0,-9mm) $) -| (strengthen-1.-25);
  \draw[->] (strengthen-1) -- node[above] {$\widehat{\xi}_1$} (bigand);
  \draw[->] (strengthen-2) -- node[below] {$\widehat{\xi}_2$} (bigand);
  \draw[->] (strengthen-n.10) -- node[below] {$\widehat{\xi}_n$} (bigand);
  \draw[->] (bigand) -- (output);

  % Redrew "strengthen" nodes to cover the lines (lol)
  \node(strengthen-2')[draw,fill=white,fill opacity=0.9] at (strengthen-2)
    { Strengthen$^{T}_{T'}$ };
  \node(strengthen-n')[draw,fill=white,fill opacity=0.9] at (strengthen-n)
    { Strengthen$^{T}_{T'}$ };
  
\end{tikzpicture}


==> gfx/cactus-plot-coverage.tex <==

% sorting in latex, works but slow
%\pgfplotstablesort[sort key=mega, sort cmp={float >}]{\hsortedmega}{data/cactus-plot-coverage.dat.txt}
%\pgfplotstablesort[sort key=megab, sort cmp={float >}]{\hsortedmegab}{data/cactus-plot-coverage.dat.txt}
%\pgfplotstablesort[sort key=max, sort cmp={float >}]{\hsortedmax}{data/cactus-plot-coverage.dat.txt}


\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[
  chart title/.style={font=\relsize{1.5}, inner sep=6pt}
  ]
  \begin{axis}[
        name=mega,
        ybar=0.05pt,
        bar width=0.2pt,
        enlarge x limits={abs = 10},
        xtick distance=100,
        %ymode=log,
        %ytick distance=10^1,
        ymajorgrids=true,
        xlabel={Benchmarks},
        ylabel={Coverage ratio},
        width=10cm,
        height=6cm]
        
    \addplot[draw=none, fill=red!80!gray]
      table[x=n,y=MeGAb] {data/cactus-plot-coverage/sorted-by-MeGAb.dat.txt};
    \addplot[draw=none, fill=blue]
      table[x=n,y=MeGA] {data/cactus-plot-coverage/sorted-by-MeGA.dat.txt};

  \end{axis}
  
  \node[chart title, at=(mega.north), anchor=north] 
    {{\color{blue}$\bullet$\,}\MEGA$-$\SMTint\hspace{.7em}%
     {\color{red}$\bullet$\,}{\MEGAb}$-$\SMTint};

  \begin{axis}[
        name=max,
        at=(mega.south east), anchor=south west,
        xshift=1cm,
        ybar,
        bar width=0.2pt,
        xmin=-10,
        xmax=450,
        xtick distance=100,
        %ymode=log,
        %ytick distance=10^1,
        ymajorgrids=true,
        xlabel={Benchmarks},
        width=10cm,
        height=6cm]
        
    \addplot[draw=none, fill=purple]
      table[x expr=\coordindex,y=max] {data/cactus-plot-coverage/sorted-by-max.dat.txt};

  \end{axis}

  \node[chart title, at=(max.north), anchor=north] {max\{\MEGA,{\MEGAb}\}$-$\SMTint};

\end{tikzpicture}%
}

==> gfx/cactus-plot-num-samples.tex <==

% sorting in latex, works but slow
%\pgfplotstablesort[sort key=mega, sort cmp={float >}]{\sortedmega}{data/cactus-plot-num-samples.dat.txt}
%\pgfplotstablesort[sort key=megab, sort cmp={float >}]{\sortedmegab}{data/cactus-plot-num-samples.dat.txt}
%\pgfplotstablesort[sort key=max, sort cmp={float >}]{\sortedmax}{data/cactus-plot-num-samples.dat.txt}



\resizebox{0.5\textwidth}{!}{%
\begin{tikzpicture}[
  chart title/.style={font=\relsize{1.5}, inner sep=6pt}
  ]
  \begin{axis}[
        name=mega,
        ybar,
        bar width=0.2pt,
        xmin=-10,
        xmax=450,
        xtick distance=100,
        ymode=log,
        ytick distance=10^1,
        ymajorgrids=true,
        minor y tick num=1,
        xlabel={Benchmarks},
        ylabel={\#\,samples ratio},
        width=10cm,
        height=6cm]
        
    \addplot[draw=none, fill=blue]
      table[x expr=\coordindex,y=MeGA] {data/cactus-plot-num-samples/sorted-by-MeGA.dat.txt};

  \end{axis}

  \node[chart title, at=(mega.north), anchor=north] {\MEGA/\SMTint};

  \begin{axis}[
        name=megab,
        at=(mega.south east), anchor=south west,
        xshift=1cm,
        ybar,
        bar width=0.2pt,
        xmin=-10,
        xmax=450,
        xtick distance=100,
        ymode=log,
        ytick distance=10^1,
        ymajorgrids=true,
        xlabel={Benchmarks},
        width=10cm,
        height=6cm]
        
    \addplot[draw=none, fill=red!80!gray]
      table[x expr=\coordindex,y=MeGAb] {data/cactus-plot-num-samples/sorted-by-MeGAb.dat.txt};

  \end{axis}

  \node[chart title, at=(megab.north), anchor=north] {\MEGAb/\SMTint};

\end{tikzpicture}%
}

==> grounding_proof.tex <==
\section{Proof of the Grounding Fidelity Lemma (\Cref{lemma:grounding_fidelity})}\label{appendix:grounding-proof}
\begin{proof}
By induction on the structure of terms $t\sqsubseteq\varphi$.
If $t$ is a select-term, then $t\in S$ and $m[t]=\agm[v_t]$ by the definition of atomic grounding.
Otherwise, $t$ is of the form $f(t_1,\ldots,t_n)$ where $f$ is an interpreted function of the theory and $t$ is not of array sort.
(Notice that subterms in $\aselect$ are never reached in this proof, and all other occurrences of arrays have been eliminated.)
Therefore the equivalence is obtained from the induction hypothesis on $t_1,\dots,t_n$ and from the fact that the interpretation of $f$ is fixed.
\end{proof}

==> intro_draft.tex <==

% SMT is useful and standard
\emph{SMT}, the \emph{satisfiability modulo theories} decision problem, is used
for many different purposes in computer science. 
For instance, one can encode the conditions under which a program exhibits a certain behavior as an SMT formula.
The solution to the satisfiability problem for that formula then indicates whether said behavior can, in fact, occur, and a model, if found, represents program inputs that trigger it.
Off-the-shelf SMT solvers are available~\cite{DeMoura:2008,Barrett:2011}, as well as a
standard set of theories, SMT-LIB~\cite{Barrett:2021}, each with its set of benchmarks.

% But we often need multiple solutions, not one
By and large, these tools are focused on generating a \emph{single}
model for a satisfiable formula.
However, there are many use cases in which multiple, even a large number of, such models are needed.
For example, for symbolic execution engines and white-box fuzzers that generate tests for a given program, it would be insufficient to have only one test case.
It is also desirable to have a variety of solutions that are representative of the solution space, \ie \emph{sample} the space with some non-zero probability for every point therein.
This paper is concerned with efficiently generating
multiple random solutions for an SMT expression with good coverage of the
constraint space.

% Introduce theories as ways to model different real-life problems
SAT sampling, dealing with Boolean constraints, is a well-studied problem in the literature; but real-world programs often contain complex objects such as integers, arrays and bit-vectors, which are better represented using first-order theories found in SMT-LIB.
% SAT sampling is studied, SMT sampling is not
While the problem of generating multiple, diverse solutions to SAT constraints has been
successfully established with techniques such as Markov Chain
Monte-Carlo~(MCMC), the history of same problem applied to SMT constraints is shorter.
The best solutions the authors are aware of are presented in \SMTSampler~\cite{Dutra:2018} and
\GuidedSampler~\cite{Dutra:2019}.

%  Why SMT is harder than SAT
The extension of Boolean formulas to theories presents multiple challenges.  
The complexity of the constraints may cause the solution space to be sparse and
unevenly distributed, making traditional techniques used for SAT inefficient or
ineffective. 
%  Another challenge- we want diversed solutions
Moreover, we would like to ensure that the generated solutions are diverse so that, \eg testing based on these samples would be effective.
Given an SMT constraint with an integer \(x\) that happens to be unconstrained, we could
easily generate many solutions that differ only in~\(x\), or some other
simple-to-explore axis, which is not always what we would be after.  
While such an approach may provide a large number of solutions, it ignores a large part of
the solution space, which may hide more faults. 
% Another challenge - generality for many theories
Yet another challenge is designing a technique that can support the various theories offered by SMT.

% 2. Model Based Under Approximation
% 2a. Outline of SMTSampler (epochs)
This work re-uses the basic overall framework of \SMTSampler.  
This framework is so-called \emph{epoch-based}: it operates in a series of rounds, called
\emph{epochs}, where in each epoch a \textit{seed} $m$, which is a random model
of the formula, is generated using an off-the-shelf~(MAX-)SMT solver.  
Then, the technique generates neighboring models that differ as little as possible from
$m$, calculates the mutation from $m$ to the neighbor, and combines several
mutations to create a set of new models.

% 2b. Instead of doing <...>, we use a simpler formula that underapproximates
% $\varphi$, \ie, implies the original formula and is easier to sample
Our approach retains the structure of epochs that begin with a seed obtained via
an SMT solver and expand it to a set of solutions.  But, rather than generate
mutations as in \SMTSampler, we derive a simpler formula, \(\hat{\varphi}\),
that underapproximates an input formula \(\varphi\), and is easier to sample.
This formula is then sampled efficiently, and the underapproximation property
ensures that every collected solution is also a solution of \(\varphi\).

% Thus, in this process of underapproximation, we in fact generalize the given solution to a set of solutions represented compactly using the formula \(\hat{\varphi}\).

We give this process of underapproximation aided by a model the name
\textit{model-guided approximation}.  We present a framework for solving
model-guided approximation problems where the formula \(\varphi\) is taken from
a first-order theory $T$ and the formula \(\hat{\varphi}\) should be taken from
a different theory, $T'$.  Our framework relies on a reduction to a simpler
case, where \(\varphi\) is a literal in $T$ (\ie an atomic formula or its
negation).  Thus, to instantiate the framework for specific theories, one needs
to provide a procedure for model-guided-approximating literals from $T$ to $T'$.


{\color{gray}
DRAFT: 
motivation for sampling (in general):
borrow from work on SAT sampling
"where a solution is useful many could be too"
if many solutions are found efficiently than one can choose the best one for a certain goal.

motivation for sampling in SMT:
SMT formulas are useful: In software verification, SMT formulas are often used to describe bad behaviors of the system [cbmc, ultimate], where a model corresponds to a bug
- having many models could help in understanding and debugging the bug, manually or automatically using test-based techniques such as [arbitrary test-based repair techniques].
[it would help to cite here also something about how the more tests the better the repair].
Also, many bug finding techniques such as symbolic execution [] and fuzzing [] rely on SMT formulas
- here, too, multiple models can help speed-up the exploration and find more bugs.

SAT sampling is not enough- SMTSAmpler showed that conversion of bitvector formulas to boolean formulas and using SAT sampling leads to way less efficient sampling.
When dealing with other domains, such as ints, it is even impossible. 

motivation for sampling Int formulas:
We present an algorithm for Ints ...
Integer theories are useful for the above-mentioned applications. 
SeaHorn, Ultimate Automizer, and Klee use Ints for reasonning about programs (do they?).
% its a good place to start :)
% int computation is efficient (in comparison to bitvectors?).
% Rules for under-approximation are easy to present and understand.
% When dealing with small ranges of numbers that do not cause overflow, or when one wants to intentionally ignore behaviors caused by overflow, Ints are the way to go.
}

==> intro_orig.tex <==
The content of this section is text from my scholarship application which we may or may not use:

The satisfiability modulo theories (SMT) solving problem is the problem of deciding satisfiability of a first-order logic formula with respect to a background theory.
The decidability and complexity of the problem is determined by the theory.
%For example, the decidability of formulas over... is exponential, while over .. is polynomial.
Over the past decade SMT solving techniques have seen unprecedented improvement that has led to its widespread use in various applications.
Presently, SMT solving plays a major role in program verification \cite{ultimate,cbmc,seahorn}, testing \cite{sage2008,klee2008}, analysis \cite{surveySE} and synthesis \cite{sketch}.
%Research nowadays focuses mainly on...

Another closely related problem is the problem of SMT sampling:
given a satisfiable SMT formula, we want to obtain as many models of it as we can.
Often it is also required that the models be diverse, or even have a uniform distribution.
This problem arises, for example, in automated testing techniques where a computer program is modeled using an SMT formula whose models correspond to execution traces of the program.
Since the goal of testing is usually to achieve large coverage of program code, multiple execution traces are needed, which correspond to multiple models of the formula.


In this work, we define the problem of model-based under-approximation of SMT formulas and introduce a method to solve it.

\begin{figure*}[t]
	\centering		
	\includegraphics[width=\textwidth]{sampling.png}
	\caption{Illustration of MBUA}
	\label{fig:samplingMBUA}
\end{figure*}

\paragraph{Model-based under-approximation (MBUA)}
An under-approximation of an SMT formula $\varphi$ is another formula, $\psi$, s.t. $\psi\implies\varphi$. 
Since every model of $\psi$ is also a model of $\varphi$, one way to obtain a model of $\varphi$ is to calculate $\psi$ and solve it instead.
Note that this strategy cannot be used to prove that $\varphi$ is not satisfiable, but in cases where $\varphi$ is satisfiable, and $\psi$ is over a theory that is easier to solve, it might pay off. 
In model-based under-approximation  (MBUA), a single model $m$ of the formula $\varphi$ needs to be present for the under-approximation to take place.
This model is then used to guide the under-approximation process, in order to obtain a satisfiable under-approximation $\psi$ (and, in particular, an under-approximation s.t. $m\models\psi$).

\paragraph{SMT sampling using MBUA}
Fig. \ref{fig:samplingMBUA} presents a scheme of our MBUA-based algorithm for SMT sampling.
The red rectangles on the left represent a set of "complex" SMT constraints, that is, constraints over a theory that is hard to solve.
Our goal is to sample these constraints, i.e., to find multiple models of their conjunction.
First, the constraints are passed to an off-the-shelf SMT solver, such as z3 \cite{z3} or Yices \cite{yices}, to obtain a single model of their conjunction.
Then, MBUA is applied based on this model, to obtain a set of "simple" constraints, that is, constraints over a theory that is easy to solve and to sample.
For example, the method we have previously developed for MBUA always returns constraints in the interval domain, where each integer variable is bounded by a constant from bellow and from above.
Solving a formula in the interval domain is straightforward: simply choose a value for each variable from in-between the given bounds. 
As a final step, the simple constraints are sampled using an off-the-shelf sampler such as SMTSampler \cite{smtsampler}, instead of the original complex constraints, which is much cheaper.
It is important to notice that MBUA guarantees by design that every model of the simple constraints is also a model of the complex ones.

\paragraph{SMT solving using MBUA}
Fig. \ref{fig:solvingMBUA} presents a scheme of our MBUA-based algorithm for SMT solving, which is based on divide-and-concur.
We begin, again, with a set of complex SMT constraints.
But, this time our purpose is to find a single model for their conjunction.
The first step is to split the original set of constraints into two sets, and solve each of them individually.
The individual solving of these two sets of constraints is much faster than solving the conjunction of all constraints, since the size of the problem is now reduced by half, and the solving problem is, in most cases, at least exponential in this size.

At this point we obtain two, most likely different, models of the two sub-problems.
Then, we use MBUA to obtain a simple set of constraints from each model.
Notice that any model of the first set of simple constraints is a model for the conjunction of the first half of complex constraints, and the same holds for the second.
At the next step, we compute the intersection of these two sets, to obtain another set of simple constraints.
MBUA should make sure that the theory used to represent simple constraints is one that is closed under intersection, and where computing the intersection is efficient.
For example, computing the intersection of two formulas in the interval domain is linear in the size of the formulas.

Finally, the simple constraints are solved using an off-the-shelf SMT solver to obtain a model.
Since this model is a model for the intersection of the two sets of simple constraints, it satisfies each of them, which means that it satisfies both parts of the original constraints.


\begin{comment}

We now introduce this problem and discuss two new methodologies, one for SMT solving and one for SMT sampling, both based on model-based under-approximation.

%We propose a new direction of progress, which is largely orthogonal to current research directions.
%While current directions focus on developing methods for solving formulas,
We propose two new methodologies, one for SMT solving and one for SMT sampling, both based on model-based under-approximation.

%Surprisingly, the SMT sampling problem has received much less attention in the literature. 


%The new methodology suggests to break a large formula into several simpler sub-formulas 
%At the basis of the new methodology is the method of endorphism that we developed as part of our doctoral work.
%This method is able to give, given one formula and one solution, a formula
%Our idea is described in Figure 1.


Some of these applications require more than one model: all, many or best.
Motivation: CRV (constrained-random-verification), fuzzing.


In poster we have presented a method for Model-guided Under-Approximation of SMT formulas.
Given a formula over the theory of LIA, and one model of it, we obtain a fomrula in the integer domain, which entails the original formula. 
This way, obtaining the next model is much easier.
In fact, for the case of the interval domain, we can now iterate over all models of the novel formula easily.


Use Refael Presentation.
We have developed a method. Only for intervals.
So far, explored its ability to enhance program repair.
Investigate what other potential it has: SMT sampling, fuzzing, faster solving (split formula, solve easy/hard part, UA, )
Also, extend to other theories (not intervals).
Iterative.
\end{comment}

==> old-framework.tex <==
\subsection{Solving the Model-Guided Approximation Problem}
{
\color{gray}

Next, we present a framework for solving the model approximation problem for two
theories $T$ and $T'$ s.t. $T'\preceq T$.  The framework is based on a reduction to a
simpler version of the model approximation problem: one where we assume the
formula $\varphi$ is a literal (i.e., an atomic formula or its negation).  We
refer to this simplified version of the model approximation problem as the
\textit{literal strengthening} problem.  Note that, while the literal
strengthening problem requires that the input formula, $\varphi$, be a literal in
$T$, it imposes no restrictions on the output formula $\hat\varphi$, which can be any
formula in $T'$.

An illustration of our framework is presented in figure~\ref{fig:framework}.
First, we collect a subset of literals $L=\xi_1,\cdots\!,\xi_n$ from $\varphi$.
Then, we make use of a black-box procedure, $Strengthen(T,T')$, for solving the
literal strengthening problem of $T$ and $T'$: each of the literals $\xi_i$ is
$m$-strengthened to obtain $\widehat\xi_i$ in $T'$.  Finally,
$\widehat\xi_1,\cdots\!,\widehat\xi_n$ are conjoined back together to form the
output formula $\hat\varphi$.

\begin{figure}[t]
    \centering
    \input{gfx/block-diagram}
    \caption{A %\SI{Do we need a name for it?} 
    framework for solving the model approximation problem of theories $T$ and $T'$}
    \label{fig:framework}
\end{figure}

In order for this process to work as expected, the subset $L$ has to satisfy
certain properties.  First, since we want all literals to be strengthened based
on the model $m$, $m$ has to satisfy all of them (this is one of the
requirements of an $m$-approximation).  Second, for $\hat\varphi$ to imply
$\varphi$, the conjunction of all literals in $L$ has to imply $\varphi$.  We
refer to a subset $L$ with these two special properties as an
\textit{\(m\)-slice} of $\varphi$:
\begin{defn}\label{def:slice}
  Let \(\varphi\) be a formula in theory \(T\), and \(m \models \varphi\).
  \(L\) is an \emph{\(m\)-slice} of \(\varphi\) iff the following holds:
  \begin{enumerate}
      \item It is a subset of literals from \(\varphi\).
      \item For every literal $\xi$ in $L$: $m \models \xi$
      \item \( \left(\bigwedge_{\xi\in L}\xi\right)\rightarrow\varphi\)
  \end{enumerate}
\end{defn}

Next, we present an algorithm for computing an {\(m\)-slice} of $\varphi$.  Our
algorithm, \texttt{ToSlice}, is listed as \cref{alg:toslice}.  It assumes the
input formula \(\varphi\) is in negation normal form (NNF), i.e., that the negation
operator is applied only to atomic formulas in \(\varphi\).
% \[\varphi: Atomic, \varphi \land \varphi, \varphi \lor \varphi, \lnot \varphi \]
This assumption is reasonable, since every formula can be converted to NNF
efficiently by propagating negation inwards, using De-Morgan laws, without
increasing the number of literals in the
formula~\cite{Book2001:Degtyarev}. 
The operation of the algorithm is split into two cases: if \(\varphi\) is a
conjunction, it returns a set of literals by applying itself recursively to each
term of the conjunction and unifying the returned sets.  Note that, $m$ indeed
satisfies each of these conjuncts, so a recursive call is possible.  Otherwise,
for disjunctions, there exists at least one term that \(m\) satisfies, so one
such term is selected at random and the rest are discarded.  Since $\varphi$ is
in NNF, the only other option is for $\varphi$ to be a literal.  In such a case,
a singleton containing only $\varphi$ itself is returned.
  
  \begin{algorithm}[t]
\footnotesize %\centering
\textbf{Input:} An NNF formula \(\varphi\), \(m\in \Models(\varphi)\) \\
\textbf{Output:} An \(m\)-slice of \(\varphi\)
\begin{algorithmic}[1]
  \If {\(\varphi\) is an \(\bigwedge\)-formula}
    \State \Return \(\bigcup_{t_\land\in\varphi}\) \texttt{ToSlice}\(\left(t_\land,m\right)\)
  \ElsIf {\(\varphi\) is an \(\bigvee\)-formula}
    \State \(D := \{t_\lor\in\varphi \mid m\models t_\lor\}\)
    \State \(t_\lor := \texttt{Random}(D)\)         \Comment{Randomly choose an element from $D$}
    \State \Return \texttt{ToSlice}\(\left(t_\lor,m\right)\)
  \Else
    \Comment{\(\varphi\) is a literal}
    \State \Return \(\{\varphi\}\)
  \EndIf
\end{algorithmic}
\caption{\texttt{ToSlice}}\label{alg:toslice}
% \vspace{-12pt}
\end{algorithm}

To sum up, the following propositions assert the correctness of the
\texttt{ToSlice} algorithm and of the framework as a whole. \BC{Do we need
  proofs?}
% Their proofs can be found in Appendix.

\begin{proposition}
  For every NNF formula $\varphi$ and every model $m$ of $\varphi$ \texttt{ToSlice} returns
  an $m$-slice of $\varphi$.
\end{proposition}

\begin{proposition}
  Given a block-box procedure $Strengthen(T,T')$ for solving the literal
  strengthening problem of $T$ and $T'$, the framework of
  \cref{fig:framework}\BC{name it?} returns for every NNF formula $\varphi$ and every
  model $m$ of $\varphi$ an $m$-approximation of $\varphi$ in $T'$.
\end{proposition}
}

==> proofs.tex <==
\subsection{Proof of~\cref{lemma:grounding_fidelity}}\label{sec:proofs}
\begin{proof}
By induction on the structure of terms $t\sqsubseteq\varphi$.
If $t$ is a select-term, then $t\in S$ and $m[t]=\agm[v_t]$ by the definition of atomic grounding.
Otherwise, $t \cong f(t_1,\ldots,t_n)$ where $f$ is an interpreted function of the theory and $t$ is not of array sort.
(Notice that subterms in $\aselect$ are never reached in this proof, and all other occurrences of arrays have been eliminated.)
Therefore the equivalence is obtained from the induction hypothesis on $t_1,\dots,t_n$ and from the fact that the interpretation of $f$ is fixed.
\end{proof}

==> sampling.tex <==

In this section, we present a framework for sampling SMT formulas in a theory $T$. 
Sampling is based on model approximation to a theory $T'$ s.t. \(T'\preceq T\), as described in \cref{sec:mbua}.
Our sampling framework, \(\texttt{MeGASample}^T_{T'}\), relies on three black-box procedures:
\begin{enumerate}
    \item \(\texttt{MAX-Solve}^T\) - for solving the MAX-satisfiability modulo $T$ problem. Such a solver enables to partition constraints into two sets, hard and soft, and the goal is to find a model that satisfies all hard constraints and a maximum number of soft constraints
    \footnote{A variant of the framework exists where only a (non-MAX) solver is required, as explained below.}.
    \item \(\texttt{PMGA}^T_{T'}\) - for solving the product model-guided approximation problem of $T$ and $T'$. 
    \item \(\texttt{Sample}_{T'}\) - for sampling formulas in $T'$.
\end{enumerate}
Note that, the choice of $T'$ should be such that there exist efficient procedures for both \(\texttt{PMGA}^T_{T'}\) and \(\texttt{Sample}_{T'}\).

\begin{figure*}
  \centering
 \input{gfx/workflow.tex}%
 \caption{Workflow of the \(\texttt{MeGASample}^T_{T'}\) sampling framework }
 \label{fig:workflow}
\end{figure*}

% \begin{algorithm}[t]
% \footnotesize %\centering
% \textbf{Input:} A formula \(\varphi\) in theory \(T\) \\
% \textbf{Output:} A set \(M\subseteq \Models\left(\varphi\right)\)
% \begin{algorithmic}[1]
%   \State \({\varphi}_{\textsc{nnf}} \coloneqq \texttt{ToNNF}\left(\varphi\right)\)
%   \State \(M \coloneqq \emptyset\), \(\hat\varphi \coloneqq false\)
%   \While {timeout not reached} \label{alg:mainloop:while}
%     \State \(m \coloneqq \texttt{GetSeed}\left(\varphi_{\textsc{nnf}},\hat\varphi\right)\) \label{alg:mainloop:getseed}
%     \Comment{Two alternatives for this procedure}
%     \State \textbf{exit if} \(m=\bot\)
%     % \Comment {No more solutions to \(\varphi\)}
%     \State \textbf{output} \(m\) \textbf{if} \(m \notin M\)
%     \State \(M \coloneqq M\cup\{m\}\)
%     \State \(\psi \coloneqq \texttt{ToSlice}\left({\varphi}_{\textsc{nnf}},
%       m\right)\) \label{alg:mainloop:toslice}
%     \Comment {c.f.~\cref{alg:toslice}}
%     \State \(\hat\varphi \coloneqq \bigwedge_{\xi\in\psi}
%     \texttt{Strengthen}_{T'}^T\left(\xi,m\right)\)\label{alg:mainloop:strength}
%     \Comment {c.f.~\cref{fig:integer-rules}}
%     \State \(\widehat M \coloneqq \texttt{Sample}\left(\hat\varphi\right)\)
%     \label{alg:mainloop:sample}
%     \State \textbf{output all} \(\hat m\in\hat M\) \textbf{if} \(\hat m\notin M\) \label{alg:mainloop:output}
%     \State \(M \coloneqq M\cup\widehat M\)
%   \EndWhile
% \end{algorithmic}
% \caption{\(\texttt{MeGASample}^T_{T'}\)}\label{alg:mainloop}
% % \vspace{-12pt}
% \end{algorithm}

Similar to~\cite{Dutra:2018}, the sampling process is \textit{epoch-based}:
it obtains an initial model with the help of a solver, and then utilizes it to create a set of distinct models in an efficient manner.
This process is repeated iteratively, where each such iteration is called \textit{an epoch}.
The initial model of each epoch is called the \textit{seed} of the epoch.

\paragraph{Framework outline}
An outline of the \(\texttt{MeGASample}^T_{T'}\) framework is presented in \cref{fig:workflow}.
As a preliminary step, the input formula $\varphi$ is transformed into negation~normal~form (NNF) in \texttt{ToNNF}, since this is a prerequisite for the subsequent \texttt{ComputeImplicant} procedure.
Conversion to NNF is done in the standard way, by propagating negation inwards using De-Morgan laws, without increasing the number of literals in the
formula~\cite{Book2001:Degtyarev}.
Then, the epoch loop begins, collecting models in the set $M$ (initialized to $\emptyset$).
First, the seed of the epoch, $m$, is obtained using the \texttt{GetSeed} procedure.
Note that, in addition to $\varphi_{NNF}$, this procedure also gets the underapproximated formula $\varphi'$ of the previous epoch, which is sometimes used to guide the choice of the seed.
% Details of this procedure are provided below.
Then, model-guided approximation takes place.
As discussed in~\cref{sec:mbua-comp}, the first step is to find a product term $P$ that is an $m$-implicant of $\varphi_{NNF}$ (and $\varphi$) in \texttt{ComputeImplicant}, in order to reduce the MGA problem to a PMGA problem.\BC{make sure these initials are consistent in all places} 
Then, the black-box \(\texttt{PMGA}^T_{T'}\) procedure is used to obtain $\varphi'$, an $m$-approximation of $P$ (and $\varphi$).
Finally, in \texttt{Exploit$\varphi'$}, the formula $\varphi'$ is repeatedly sampled with the help of \(\texttt{Sample}_{T'}\), and its set of models, $M'$, is returned.
Note that, the \(m\)-approximation property guarantees that every model of \(\varphi'\) is also a model of \(\varphi\).
Therefore, all models in $M'$ are output if they were not seen before (\ie not in $M$), and the set $M$ is updated accordingly.

\paragraph{The \texttt{GetSeed} procedure}
For the \texttt{GetSeed} procedure, we consider two variants: random-based and blocking-based.
The random-based variant is taken from~\cite{Dutra:2018}. 
It selects an assignment at random and finds the closest model to it by adding $\varphi$ to \(\texttt{MAX-Solve}^T\) as a hard constraint, and the equivalence to the assignment as a set of soft constraints.
The blocking-based variant attempts to find unseen solutions by discarding all models of the underapproximated formulas obtained in previous epochs.
It adds $\varphi$ to \(\texttt{MAX-Solve}^T\) as a hard constraint and the negation of the underapproximated formula $\hat\varphi$ of the previous iteration as a soft constraint.
Unlike the random-based variant, soft constraints are accumulated between different calls to the solver, to enable blocking based on the entire history of epochs.

\paragraph{The \texttt{ComputeImplicant} procedure}
Several algorithms exist for computing all prime implicants of $\varphi$ \cite{Coudert_Madre_Jaures_1993,Jackson_Pais_1990,Slagle_Chang_Lee_1970,Strzemecki_1992}.
However, we only need to find one implicant of $\varphi$ that need not be prime, but has to be satisfied by $m$.\BC{define prime just to say we don't care about it?}
Therefore, we follow this simple procedure:
Assuming the formula was a-priori converted to NNF, we traverse its abstract-syntax-tree in a top-down fashion, and from each disjunction we leave only one disjunct that is chosen randomly from all disjuncts satisfied by $m$.
The top-down order ensures that $m$ satisfies every sub-formula we encounter. 
This, in turn, ensures that for every disjunction we encounter there exists at least one disjunct satisfied by $m$.
It also ensures that every literal in the returned product term is satisfied by $m$.
\BC{Do we need the algorithm? proof? proof sketch? or is this enough?}
\BC{go back to the review and the Yices reference and see if a citation is needed}

\paragraph{The \texttt{Exploit$\varphi'$} procedure}
A simple implementation of the \texttt{Exploit$\varphi'$} procedure is to simply use \(\texttt{Sample}_{T'}\) out of the box. 
However, to avoid wasting time sampling a formula $\varphi'$ with very few new solutions, we perform \(n\) sampling rounds in which \(m\) randomly-drawn samples are produced using \(\texttt{Sample}_{T'}\). 
After finishing each round, if the rate of unique new samples generated falls under a
predefined limit, the sampling of this formula is stopped. 
Additionally, one can heuristically adjust \(m\) and \(n\) based on properties of the formula $\varphi'$.\BC{if this goes in the appendix we should provide more details here}

\paragraph{Instantiation for integer theories}
Next, we instantiate the \(\texttt{MeGASample}^T_{T'}\) framework for two pairs of theories: $T=\Tmia,T'=\Tic$ and $T=\Tamia,T'=\Taic$.
Both instantiations utilize an off-the-shelf MAX-SMT solver in the role of $\texttt{MAX-Solve}^T$.
In the role of \(\texttt{PMGA}^T_{T'}\), the former uses the algorithm from~\cref{subsec:rules} and the later uses the algorithm from~\cref{sec:arrays}.
As per \(\texttt{Sample}_{T'}\), for $T'=\Tic$ this procedure can be realized by repeatedly drawing a value at random from within the lower and higher bounds of each variable for each sample. 
For $T'=\Taic$, things get a little more complicated since we need to also sample array elements constrained by an interval.
As already mentioned in~\cref{sec:arrays}, clashes may occur between terms that are not syntactically identical but refer to the same array element (are aliased).
We can use a generate-and-test approach on top of the $\Tic$ sampling procedure (reference implementation is shown in~\cref{alg:sampleaic}).
However, we have already shown that with the addition of equality and inequality constraints we can eliminate aliasing a-priori. 
We therefore use the $\Tic$ sampling procedure also for $\Taic$.


%%% Local Variables:
%%% mode: latex
%%% coding: utf-8
%%% TeX-master: "main"
%%% TeX-PDF-mode: t
%%% TeX-engine: default
%%% End:


==> technical-details.tex <==

\section{Technical Details of \MeGASampler}\label{appendix:technical-details}

\paragraph{The \texttt{GetSeed} procedure}
For the \texttt{GetSeed} procedure, we consider two variants: random-based and blocking-based.
The random-based variant is taken from~\cite{Dutra:2018}. 
It selects an assignment at random and finds the closest model to it by adding $\varphi$ to \(\texttt{MAX-Solve}^T\) as a hard constraint, and the equivalence to the assignment as a set of soft constraints.
The blocking-based variant attempts to find unseen solutions by discarding all models of the underapproximated formulas obtained in previous epochs.
% It adds $\varphi$ to \(\texttt{MAX-Solve}^T\) as a hard constraint and the negation of the underapproximated formula $\hat\varphi$ of the previous iteration as a soft constraint.
It does that by adding the negation of the underapproximated formula $\hat\varphi$ from previous iterations to \(\texttt{MAX-Solve}^T\) as a hard constraint.
In fact, since this variant only makes use of hard constraints, it replaces \(\texttt{MAX-Solve}^T\) with \(\texttt{Solve}^T\), which is more efficient than \(\texttt{Solve}^T\).
Unlike the random-based variant, constraints are accumulated between different calls to the solver, to enable blocking based on the entire history of epochs. 
If at some point the solver fails to find a solution, all the constraints are removed and the process starts anew.

\paragraph{The \texttt{Exploit$\varphi'$} procedure}
A simple implementation of the \texttt{Exploit$\varphi'$} procedure is to simply use \(\texttt{Sample}_{T'}\) out of the box. 
However, to avoid wasting time sampling a formula $\varphi'$ with very few new solutions, we perform \(n\) sampling rounds in which \(m\) randomly-drawn samples are produced using \(\texttt{Sample}_{T'}\). 
After finishing each round, if the rate of unique new samples generated falls under a
predefined limit, the sampling of this formula is stopped. 
Additionally, one can heuristically adjust \(m\) and \(n\) based on properties of the formula $\varphi'$.\BC{if this goes in the appendix we should provide more details here}

\paragraph{The \(\texttt{Sample}_{T'}\) procedure for \(T'=\Taic\)}
\begin{algorithm}[t]
\footnotesize %\centering
\textbf{Input:} A formula \(\varphi\) in \(\Taic\) represented using a map $IM^\varphi$ from terms to intervals\\
\textbf{Output:} A set \(M\subseteq \Models\left(\varphi\right)\)
\begin{algorithmic}[1]
  \State \(M := \emptyset\)
  \While {timeout not reached}
    \State \(m\) := \(\emptymodel\)                 
    \State validModel := true
    \For {\(v\in IM^\varphi\) \textbf{if} \(v\) is an int variable}
        \State \(m\) := \(\miassign{m}{v}{Random(IM^\varphi[v])}\) \Comment{draws a random value from the interval}
    \EndFor
    \For {\(t\in IM^\varphi\) \textbf{if} \(t=select(a,i)\) \textbf{in increasing order} of selects in \(i\)}
        \State \(i_{val}\) := \(evalWithModelCompletion(m, i)\)
        \If {\(\maeval{m}{a}{i_{val}} \neq \bot \)}
            \If {\(\maeval{m}{a}{i_{val}} \notin IM^{\varphi}[t]\)}
                \State validModel := false
                \State \textbf{break} \Comment{move on to the next \(m\)}
            \EndIf
        \Else
            \State \(m\) := \(\maassign{m}{a}{i_{val}}{Random(IM^\varphi[t])}\)
        \EndIf
    \EndFor
    \If{validModel}
        \State \(M\) := \(M\cup \{m\}\)
    \EndIf
  \EndWhile
  \State \textbf{return} \(M\)
\end{algorithmic}
\caption{\(\texttt{Sample}_{\Taic}\)}\label{alg:sampleaic}
\end{algorithm}

\cref{alg:sampleaic} presents an algorithm for sampling formulas in $\Taic$.
This algorithm gets a formula \(\varphi\) in \(\Taic\) and returns a set \(M\subseteq \Models\left(\varphi\right)\).
Since every formula in $\Taic$ is in fact a conjunction of intervals over select-terms and integer variables, the formula can be represented using a map $IM^\varphi$ from terms to intervals.

The algorithm uses the notation \(\miassign{m}{v}{c}\), where $v$ is an integer variable symbol and $c$ is an integer value, to denote the model $m$ with the value of $v$ set to $c$. 
Similarly, \(\maassign{m}{a}{i}{e}\), where $a$ is an array variable symbol and $i,e$ are integer values, denotes the model $m$ with the value of $a$ (a function) set to map $i$ to $e$.
The notation $\bot$ denotes the empty model, where none of the variables is assigned.
Similarly, if $m[v]$, for some variable $v$, equals $\bot$, then $v$ is not set in $m$.

The algorithm begins by initializing the constructed model $m$ to $\bot$. 
Then, the values of all integer variables that are constrained by an interval is determined by randomly sampling a value for each variable $v$ from its interval $IM^\varphi(v)$.
Next, select-terms of the form \(t=select(a,i)\) are considered.
Initially, the value of the index term $i$ is fixed and saved in $i_{val}$ using the \texttt{evalWithModelCompletion} procedure.
This procedure checks if $i$ was already set in $m$, and if not, sets it to some random value.
Then, we check if the function $m[a]$ already maps the value $i_{val}$ to some value (\ie if array $a$ already has a value in index $i_{val}$).
This could happen if for a previous select-term \(t'=select(a,j)\), the value of $j_{val}$ was equal to $i_{val}$. 
If this is indeed the case, we check if, by chance, the value assigned to $m[a](i_{val})$ is in the interval required for $t$.
If not, then the model $m$ cannot be completed to a valid model, and its construction is stopped\footnote{In our use of this algorithm we make sure this case is never reached by implicitly adding constraints to $\varphi$ to avoid it.}.
If $m[a](i_{val})$ was not previously assigned, then a random value from the interval of $t$ is chosen for it.
Finally, if completed successfully, the model $m$ is added to the output set $M$.

